GARLIC: GPT-Augmented Reinforcement Learning with Intelligent Control for Vehicle Dispatching

As urban residents demand higher travel quality, vehicle dispatch has become a critical component of online ride-hailing services. However, current vehicle dispatch systems struggle to navigate the complexities of urban traffic dynamics, including unpredictable traffic conditions, diverse driver behaviors, and fluctuating supply and demand patterns. These challenges have resulted in travel difficulties for passengers in certain areas, while many drivers in other areas are unable to secure orders, leading to a decline in the overall quality of urban transportation services. To address these issues, this paper introduces GARLIC: a framework of GPT-Augmented Reinforcement Learning with Intelligent Control for vehicle dispatching. GARLIC utilizes multiview graphs to capture hierarchical traffic states, and learns a dynamic reward function that accounts for individual driving behaviors. The framework further integrates a GPT model trained with a custom loss function to enable high-precision predictions and optimize dispatching policies in real-world scenarios. Experiments conducted on two real-world datasets demonstrate that GARLIC effectively aligns with driver behaviors while reducing the empty load rate of vehicles.

==> 999Checklist.tex <==
\section{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\noindent This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \bl{Yes.}

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: \bl{Yes.}

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \bl{Yes.}
\end{itemize}

\noindent Does this paper make theoretical contributions?: \bl{No.}

\noindent If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

    \item Proofs of all novel claims are included. (yes/partial/no)

    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)

    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)

    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\noindent Does this paper rely on one or more datasets? \bl{Yes.}

\noindent If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets: \bl{Yes.}

    \item All novel datasets introduced in this paper are included in a data appendix: \bl{Yes.}

    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: \bl{Yes. If the paper is accepted, we would like to share all the datasets used in this paper through academic collaboration.}

    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations: \bl{Yes.}

    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available: \bl{Yes.}

    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing: \bl{Yes.}
\end{itemize}


\noindent Does this paper include computational experiments? \bl{Yes.}

\noindent If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix: \bl{Yes.}
    
    \item All source code required for conducting and analyzing the experiments is included in a code appendix: \bl{Yes.}
    
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: \bl{Yes.}
    
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from: \bl{Yes.}
    
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results: \bl{Yes}
    
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks: \bl{Yes.}
    
    \item This paper formally describes the evaluation metrics used and explains the motivation for choosing these metrics: \bl{Yes.}

    \item This paper states the number of algorithm runs used to compute each reported result: \bl{Yes.}

    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information: \bl{Yes.}

    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank): \bl{Yes.}

    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments: \bl{Yes.}

    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting: \bl{Yes.}
\end{itemize}


==> draw/exp_heatacc.tex <==
\begin{figure*}[htb!]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/heat.png}
    % \vspace{-6mm}
    \caption{Supply-and-demand accuracy of hierarchical traffic state representation: The bluer the grid, the higher the accuracy.}
    \label{fig:pretrain_acc}
\end{figure*}
